OOD Aware Supervised Contrastive Learning

Out-of-Distribution (OOD) detection is a crucial problem for the safe deployment of machine learning models identifying samples that fall outside of the training distribution, i.e. in-distribution data (ID). Most OOD works focus on the classification models trained with Cross Entropy (CE) and attempt to fix its inherent issues. In this work we leverage powerful representation learned with Supervised Contrastive (SupCon) training and propose a holistic approach to learn a classifier robust to OOD data. We extend SupCon loss with two additional contrast terms. The first term pushes auxiliary OOD representations away from ID representations without imposing any constraints on similarities among auxiliary data. The second term pushes OOD features far from the existing class prototypes, while pushing ID representations closer to their corresponding class prototype. When auxiliary OOD data is not available, we propose feature mixing techniques to efficiently generate pseudo-OOD features. Our solution is simple and efficient and acts as a natural extension of the closed-set supervised contrastive representation learning. We compare against different OOD detection methods on the common benchmarks and show state-of-the-art results.

==> sections/experiments-old.tex <==
\section{Experiments}\label{sec:experiments}
In this section we provide an empirical evaluation on the proposed method, both with real and fake \OOD data, and compare it against various state-of-the-art methods.  We further ablate the main components of our contrastive training. In order to have a fair comparison with the previous literature, we adapt our settings to the unified scheme proposed in \cite{yang2022openood} and compare our performance with the results reported in this study. 
% energy: For other works not mentioned in \cite{yang2022openood}, we modify the methods and train them under a similar setting.

In particular, all methods reported in this section employ a ResNet18~\cite{he2016deep} backbone and use CIFAR-10 and CIFAR-100 \cite{krizhevsky2009learning} as the in-distribution datasets. Unless mentioned otherwise, we train our models with a batch size of 512 for 100 epochs using SGD as the optimizer and a cosine annealing scheduler \cite{loshchilov2016sgdr}.

% In the supplementary material we provide further results, using ResNet50 as the feature extractor. 
%\textbf{OOD dataset for training:}
%Throughout the experiments, we
% The Tiny Images dataset \cite{le2015tiny} is used whenever there is a requirement for real \OOD examples during training to which we remove any class intersection with either CIFAR-10 or CIFAR-100.  In the supplement we provide additional results by training our method with different \OOD data.



We extensively evaluate and report our results on Describable Textures Dataset (DTD) \cite{cimpoi2014describing}, SVHN \cite{netzer2011reading}, Places365 \cite{zhou2017places}, LSUN-Crop, LSUN-Resize \cite{yu2015lsun}, iSUN \cite{xu2015turkergaze}, iNaturalist \cite{van2018inaturalist}, Mnist \cite{deng2012mnist} and Tiny Imagenet (TIN) \cite{le2015tiny} datasets. Additionally, we evaluate our method on CIFAR-10 and CIFAR-100 datasets for the experiments that do not use the examples from these datasets during training time. We provide a brief overview of each  dataset as well as the metrics used to evaluate the methods in the sequel.

\subsection{Datasets and Metrics}

\noindent\textbf {CIFAR-10 and CIFAR-100} datasets \cite{krizhevsky2009learning} are commonly used as a benchmark for classification methods. They contain 50k training and 10k test images categorized into 10 and 100 classes respectively. 

\noindent\textbf{DTD} \cite{cimpoi2014describing} is a dataset of over 5k images of textural patterns divided into 47 categories.  %This dataset is far-OOD to all previously discussed datasets.


\noindent\textbf{SVHN} dataset \cite{netzer2011reading}  contains real world house numbers which are similarly categorized into 10 classes of digits for over 70k training and over 26k test images. %is a near-OOD dataset for Mnist since it

\noindent\textbf{Places365} dataset \cite{zhou2017places} contains over 35k test images from 365 scene categories. %This is a far-OOD dataset to CIFAR-10 and CIFAR-100 datasets.


\noindent\textbf{LSUN} (Large Scale image Understanding) dataset \cite{yu2015lsun} contains around one million labeled images, divided into 10 scene and 20 object categories. Images in the LSUN dataset have varying sizes with the smaller dimension being always 256. We use two variations of the LSUN dataset. 

\noindent\textbf{LSUN-C} crops LSUN images into random $32\times32$ patches. \textbf{LSUN-R} resizes each image to $32\times32$.

\noindent\textbf{iSUN} \cite{xu2015turkergaze} is a large-scale dataset containing saliency maps annotated from natural scene images in the SUN dataset \cite{xiao2010sun} using eye-tracking. The collection is partitioned into 6k images for training, 926 for validation and 2k for test.


\noindent\textbf{iNaturalist} \cite{van2018inaturalist} is a highly imbalanced dataset with differing number of images per category. It contains over 675k training and validation images from 13 natural super-categories such as plants, insects, birds and mammals.

\noindent\textbf{Mnist} dataset \cite{deng2012mnist} contains 60k training and 10k test images of hand-written digits categorized into 10 classes. %Mnist is considered as a far-OOD dataset for CIFAR-10 and CIFAR-100 due to their different nature of inputs and labels. 

\noindent\textbf{Tiny Imagenet (TIN)} \cite{le2015tiny} is a subset of the ImageNet dataset containing 100k images evenly split into 200 categories and resized to 64×64.


%\noindent\textbf{SUN50} is the subset of 10k images from the SUN dataset provided by \cite{sun2021react}.

% \noindent\textbf{80 Million Tiny Images (TIM)} consist of $32\times32$ images acquired from the web. Each image is taken using a non-abstract english noun in the Wordnet database \cite{miller1995wordnet}.






\noindent The metrics used to evaluate our experiments are :

\noindent\textbf{FPR@95 ($\downarrow$)},  measures the false positive rate when true positive rate is set to $95\%$, and referred to as \FPR. 

\noindent\textbf{\AUROC ($\uparrow$)},  the area under the Receiver Operating Characteristic (ROC) curve; denoting TPR/FPR relationship.

\noindent\textbf{\AUPR ($\uparrow$)}, the area under the Precision-Recall (PR) curve.
We consider \ID samples as positives.

\subsection{Compared methods}\label{sec:compared_methods}
We compare the proposed method with representative state-of the-art methods.


\myparagraph{Post hoc methods.}
\noindent\texttt{MSP}~\cite{hendrycks2016baseline} uses the maximum Softmax probability as a scoring function, a standard baseline in \OOD detection literature. 
\noindent \texttt{ODIN}~\cite{liang2017enhancing} performs perturbation in the input image and uses the MSP score on the perturbed image.
\noindent \texttt{ReAct}~\cite{sun2021react} performs a rectification on the logits for computing the \OOD detection score, here energy score is used. 

\myparagraph{Training-based methods.}
\noindent\texttt{CSI}~\cite{tack2020csi}, close to our work, leverages supervised contrastive learning. However, as a proxy for \OOD data, the method leverages strongly augmented samples.
\noindent\texttt{ARPL}~\cite{Chen2021} proposes the concept of reciprocal points as representatives for \OOD data, and train the neural network such that the features of \ID classes lie within a margin distance from those points. 
\noindent\texttt{VOS}~\cite{du2022vos} synthesizes outliers in the penultimate layer, by assuming that \ID features follow a normal distribution within each class.
\noindent \texttt{LNorm}~\cite{wei2022mitigating} trains the network such that the logits norm is constrained to be a constant. 

\myparagraph{\OOD-leveraging methods.}
\noindent\texttt{OE}~\cite{hendrycks2018deep} makes use of \CE for \ID data.
For \OOD, they set an uniform distribution as the target. 
\noindent\texttt{UDG}~\cite{yang2021semantically} leverages unsupervised data for both \OOD training and enhancing \ID performance.
Two heads are proposed.
The first one minimizes \CE loss on \ID labeled data and maximizes the entropy on \OOD data.
The second performs deep clustering.

\noindent\texttt{Energy}~\cite{liu2020energy} creates an energy gap between the ID and OOD samples. First, the mean energy values on the ID (\textit{$m_{in}$}) and OOD (\textit{$m_{out}$}) datasets are calculated.  Next, the model is finetuned to produce energy values higher than \textit{$m_{in}$} for the ID samples and lower than \textit{$m_{out}$} for OOD samples. This model achieves the best OOD detection performance compared to the other discussed methods. However, it requires an extra step for calculating the cut-off thresholds \textit{$m_{in}$} and \textit{$m_{out}$}.

\myparagraph{Our method.}
We refer to our method as \ours: OOD-aware Prototypical Supervised Contrastive learning.
Throughout the experiments we consider different variants of our method.
\textbf{\SupTT} refers to the combination of supervised contrastive training loss~\eqref{eq:supcon} with the prototypes learning loss~\eqref{eq:tt}, \OOD regularization is not applied here. 
\textbf{\oursreal} refers to models trained with our complete loss~\eqref{eq:final_loss} based on real auxiliary \OOD data.
\textbf{\oursfake} refers to models trained with our complete loss~\eqref{eq:final_loss}, here we generate \OOD-like features from \ID using~\eqref{eq:mixup} as described in Section~\ref{subsec:aux}.

We use Maximum Logit~\cite{hendrycks2019scaling} as a scoring function.
Logit here refers to the  dot product between a sample representation and a given prototype.

We further ablate different variations of our method by combining them with the finetuning scheme defined in \cite{liu2020energy}. We denote those experiments with an extra \textit{(Energy)} term added to the method's name.

\subsection{\SupTT \OOD detection performance}
We first compare the \OOD detection performance of the prototype classifier, trained with \SupCon and the tightness term (\SupTT), to a classifier trained with a cross-entropy (\CE) loss.
For fair comparison, we limit the data augmentation applied for \SupTT to standard crop, horizontal flip, and colour-jitter augmentations.\todo{Todo: remove this and change results}
We apply the same augmentations for \CE. 
Detailed results can be found in tables~\ref{tab:baselines_cifar10} and~\ref{tab:baselines_cifar100}.
We see that \SupTT consistently outperforms \CE on CIFAR-10, also improving \FPR on CIFAR-100 by a significant margin, while being comparable for \AUROC and \AUPR.
\FPR is an especially relevant metric for the purpose of rejecting \OOD samples, as it is the metric where the detection threshold is fixed, only allowing a rejection rate of $5\%$.
Achieving a lower \FPR is crucial for real life applications, where it is not possible to know the threshold in advance. 

% Our \OOD-aware training scheme succeeds in further reducing the \FPR by [ADD A NUMBER]. Note that by just using feature augmentation technique to generate pseudo-\OOD samples the \OOD detection performance improved consistently, as shown in tables \ref{tab:supt_ce_CIFAR10} and \ref{tab:supt_ce_CIFAR100}. We detail the experimental results when finetuning the model with \OOD data in the next subsection.
\input{tables/baselines-cifar10}
\input{tables/baselines-cifar100}

\setstackgap{L}{\tmp}

%CIFAR10-SUPTT-Comparison to previous
%\subsection{SupConTT vs previous work}

%\begin{table*}
%\begin{center}
%\begin{tabular}{|l|l|l|l|l|}
%\hline
%Dataset/\Longunderstack{Method \\ Metrics \\} & %\multicolumn{1}{|c|}{\Longunderstack{MSP\cite{hendryc%ks2016baseline}}} & %\multicolumn{1}{|c|}{\Longunderstack{ODIN\cite{liang2%017enhancing}}} & %\multicolumn{1}{|c|}{\Longunderstack{ReAct\cite{sun20%21react}}} & \multicolumn{1}{|c|}{\Longunderstack{Sup%TT (ours)}}\\
%\hline
%DTD & 88.72 & 80.70 & 88.18 & \textbf{96.36} \\
%\hline
%SVHN & 90.88 & 73.32 & 89.50 & \textbf{99.50} \\
%\hline
%Places365 & 89.03 & 82.55 & 90.09 & \textbf{93.52} \\
%\hline
%Mnist & 89.91 & 90.91 & 88.34 & \textbf{97.93} \\
%\hline
%CIFAR-100 & 87.11 & 77.68 & 86.35 & \textbf{91.78} \\
%\hline
%TIN & 86.62 & 77.33 & 88.90 & \textbf{92.74} \\
%\hline
%Average & 88.71 & 80.41 & 88.56 & \textbf{95.30}\\
%\hline
%\end{tabular}
%\caption {\textbf{SupTT vs previous works on %CIFAR-10:} Our method consistently produces higher %\AUROC($\uparrow$) values compared to other post-hoc %methods on different benchmark datasets.}
%\label{tab:supt_ce_cifar10}
%\end{center}
%\end{table*}


%CIFAR100-SUPTT-Comparison to previous

%\begin{table*}
%%\begin{center}
%\begin{tabular}{|l|l|l|l|l|}
%\hline
%Dataset/\Longunderstack{Method \\ Metrics \\} & %\multicolumn{1}{|c|}{\Longunderstack{MSP\cite{hendryc%ks2016baseline}}} & %\multicolumn{1}{|c|}{\Longunderstack{ODIN\cite{liang2%017enhancing}}} & %\multicolumn{1}{|c|}{\Longunderstack{ReAct\cite{sun20%21react}}} & \multicolumn{1}{|c|}{\Longunderstack{Sup%TT (ours)}}\\
%%DTD & 76.93 & 79.39 & \textbf{83.73} & 78.71 \\
%\hline
%SVHN & 76.04 & 71.08 & 71.32 & \textbf{83.54} \\
%\hline
%Places365 & 79.44 & \textbf{79.83} & 79.63 & 78.80 \\
%\hline
%Mnist & 77.78  & \textbf{83.71} & 77.02 & 65.03 \\
%\hline
%CIFAR-10 & \textbf{78.31} & 78.18 & 76.98 & 69.22 \\
%\hline
%TIN & 81.78 & 81.39 & \textbf{81.96} & 80.12 \\
%\hline
%Average & 78.38 & 78.93 & 78.44 & 75.90 \\
%\hline
%\end{tabular}
%\caption {\textbf{SupTT vs previous works on %CIFAR-100:} }
%\label{tab:supt_ce_cifar10}
%\end{center}
%\end{table*}


\subsection{OOD-Aware Supervised Contrastive Learning}
% The training scheme consider
The general form of the proposed loss function (\ref{eq:final_loss}) permits the different terms to be applied at different stages, as required by different use cases. We first train our the model with SupCon~\cite{khosla2020supervised}.
Then we fine-tune the model with our full objective function~\eqref{eq:final_loss} for additional $50$~epochs.
This allows to first learn good initial representation of the task at hand then fine-tune these representation to permit a strong separation of ID and OOD data. This also gives the possibility to fine-tune any pretrained model when \OOD data becomes available. 
We use $\gamma=1$ for training with real~\OOD and $\gamma=0.5$ for fake~\OOD.
The weight of the classification loss $\mathcal{L}_E^P +
 \mathcal{L}_E^O$ is set to $\alpha=0.1$.
 We report the mean of each metric over five different runs. 
 Here, we use the same data augmentation as in \SupCon~\cite{khosla2020supervised}, namely AutoAugment, which slightly boosts the \ID performance.
 
% Additional results, with full loss from scratch, in the supplement.
% We provide additional results in the supplement, where we report the detection performance when training with our full loss from scratch.
% 
A number of studies fine-tune their model using auxiliary data taken from a dataset \cite{hendrycks2018deep, yu2019unsupervised, yang2021semantically} different from the \InDistribution data. On the other hand, other works synthesize the auxiliary examples from the accessible ID dataset \cite{tack2020csi, chen2021adversarial, huang2021mos, du2022vos, wei2022mitigating}. Next, we compare our method to both lines of work.
\subsubsection{\todo{Comparison with SOTA OOD Training}}
Here we compare our proposed OOD training scheme with energy finetuning\cite{liu2020energy}. This method shows state of the art performance when finetuning a pretrained model with real auxiliary OOD data. Energy finetuning was originally introduced with models trained with cross entropy loss, here we investiage whether energy finetuning on top of PSupCon model is beneficial compared to our proposed OOD training scheme with real and pseudo OOD data.
\subsubsection{\todo{Comparison various SOTA methods}}
Here we compare different method of different lines as described in Sec.
We follow the evaluation protocol of \cite{loshchilov2016sgdr} by training for 100 epochs only. Note that this is suboptimal for our methods based on supervised contrastive training as it usually requires more time to converge.
In particular, all methods reported in this section employ a ResNet18~\cite{he2016deep} backbone and use CIFAR-10 and CIFAR-100 \cite{krizhevsky2009learning} as the in-distribution datasets. Unless mentioned otherwise, we train our models with a batch size of 512 for 100 epochs using SGD as the optimizer and a cosine annealing scheduler \cite{loshchilov2016sgdr}.

\subsubsection{Training with real~\OOD}
 % The question of which OOD dataset to deploy relates to the expected generalization on other OOD datasets and how much representative this OOD dataset  of all other possible OOD data. We show that our proposed contrastive training scheme can generalize to other OOD datasets without accessing a dataset with specific OOD objects, we use  DTD dataset\cite{cimpoi2014describing}; a collection of various textures. In principle such dataset can be synthetically generated using state of the generation techniques. Existing outlier exposure works~\cite{hendrycks2018deep, liu2020energy} leverage TinyImages\cite{le2015tiny}, a dataset of 8 milion images of different objects. This acts as an extensive set of all other possible objects. This dataset is not publicly available anymore, we also show the performance of our method when accessing TinyImageNet dataset, a small subset of ImageNet (100 classes). 
Typically the~\OOD data used for training should optimally cover and represent a large spectrum ranging from near-\OOD to far-\OOD examples.
Auxiliary dataset deployed before in~\cite{hendrycks2018deep, liu2020energy}  is  a large diverse dataset, \ie, TinyImages, a dataset of 8 million images of various objects, which acts as an extensive set of all other possible objects.
This dataset is not publicly available anymore.
In our work, we show that our proposed contrastive training scheme can generalize to other \OOD datasets without accessing a huge dataset with various types of \OOD objects \todo{Do we need to stress this given that we have trained energy similarly?}.
We use DTD dataset~\cite{cimpoi2014describing}, a collection of various textures.
In principle such dataset can be synthetically generated using state-of-the-art generation techniques.
We also show the performance of our method when accessing TinyImageNet dataset, a small subset of ImageNet (200 classes) in section~\ref{TIN-training}. 

% We use Tinyimages (TIM) dataset for training with real \OOD data while taking out the indices that are similar to the examples in the CIFAR dataset.

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.15\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/placeholder.png}
%          \caption{TIM dog sample}
%          \label{fig:TIM-dog-sample}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.15\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/placeholder.png}
%          \caption{TIM dog sample}
%          \label{fig:CIFAR-10-dog-sample}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.15\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/placeholder.png}
%          \caption{TIM dog sample}
%          \label{fig:CIFAR-100-dog-sample}
%      \end{subfigure}
%         \caption{Example}
%         \label{fig:three graphs}
% \end{figure}

Tables \ref{tab:sota_comparison_cifar10} and \ref{tab:sota_comparison_cifar100} show \OOD detection performance on CIFAR-10 and CIFAR-100. Our \oursreal \todo{Maybe we can limit the name to OpSupCon-R} outperforms state of the art methods from different families reducing the \FPR rate by $11.96$ on CIFAR-10 and $18.67$ on CIFAR-100.
These results suggests the effectiveness of our training pipeline when leveraging real auxiliary \OOD data.

\input{tables/cifar10}
\input{tables/cifar100}

\subsubsection{Training with pseudo-\OOD}
Selecting a dataset as \OOD is an ambiguous task dependent on the \ID data.
Previously, we showed that a dataset of different textures is sufficient to improve the \OOD detection performance on the examined \OOD datasets.
We further provide a simple alternative strategy to mimic \OOD like features as described in Section~\ref{subsec:aux}.
%It might be difficult to find a universally optimal \OOD dataset due to the scarcity of \OOD data or overlaps in the distribution, context and class categories of the \InDistribution and potential \OOD datasets.

% Building on the observation we imitate such \OOD examples using the techniques . 
We compare our method's performance (\oursfake) to previous work that synthesize \OOD data using the \ID dataset in table \ref{tab:sota_comparison_cifar10} and \ref{tab:sota_comparison_cifar100} for CIFAR-10 and CIFAR-100 benchmarks respectively.
We show that our general loss formulation can benefit from \OOD-like features and supersede the rival state of the art methods which leverage real-\OOD data thanks to the powerful representation training mechanism.
In the supplementary materials we show that further combining fake and real \OOD data can provide an extra boost to the detection performance.
%\oursfake achieves the best average AUROC on CIFAR-10 (96.57) and on CIFAR-100 (82.85).

\subsubsection{Finetuning with \texttt{Energy}~\cite{liu2020energy}}
We further finetune different models presented in tables~\ref{tab:baselines_cifar10} and~\ref{tab:baselines_cifar100} with the method proposed in ~\cite{liu2020energy} and investigate their performance, denoted with \textit{(Energy)} in the tables. 

This method requires an extra step to determine cut-off thresholds \textit{$m_{in}$} and \textit{$m_{out}$} for each model. We find that these cut-offs are very close for the models trained with a SupCon loss and thus do not provide the required energy gap between ID and OOD samples intended in this work. We fix this issue by scaling the prototype classifier weights. Note that a scaling factor would not affect the classification accuracy of (O)PSupCon models since the \textit{cosine similarity} of each sample's features to the prototypes stays the same. However, a scaling factor larger than 1 would increase the margin between the mean energy values for the ID and OOD samples a.k.a \textit{$m_{in}$} and \textit{$m_{out}$}. However, we find that assigning very large scale factors and thus a large energy gap would decrease the classification accuracy and the OOD performance after the finetuning step (See supplementary material for the ablation).

As illustrated in tables \ref{tab:baselines_cifar10} and~\ref{tab:baselines_cifar100}, even with the right scaling factors, our method does not benefit much from the finetuning paradigm proposed in \cite{liu2020energy}. Besides, (O)PSupCon variations without the energy finetuning surpass the performance of the Cross-Entropy classifier proposed in \cite{liu2020energy} and set new state-of-the-art for OOD detection.

\subsubsection{Effect on \ID classification Accuracy}
\input{tables/classification_accuracies}
Our proposed approach combines a prototypical classifier as opposed to a cross entropy trained classifier.
This is in addition to the regularized \OOD training.
Table~\ref{tab:cs_ac} reports the classification performance in terms of Accuracy for \CE, \SupTT, \oursreal and \oursfake.
It can be seen that all variants improve over \CE training thanks the powerful supervised contrastive training objective.
On CIFAR-10, all  variants perform similarly, interestingly, our \OOD regularization improves slightly the accuracy on CIFAR-100. 
\subsubsection{Effect of the choice of Auxiliary \OOD Data  } \label{TIN-training}
\input{tables/timVSsun50}
Our approach regularizes the training with \OOD specific losses. This section investigates the effect of the chosen \OOD dataset. In the main experiments, we consider DTD and textures dataset.
For comparison, we test \oursreal with TIN dataset, a dataset similar in nature to CIFAR-10 or CIFAR-100 combining 200 different object categories.
Table~\ref{tab:timsun} reports the OOD detection performance on different \OOD datasets for CIFAR-10 as an \ID task.
Depending on the \OOD dataset being evaluated, \OOD training with one dataset can improve over the other.
This is probably related to what extent the deployed auxiliary \OOD data is similar to the test \OOD data.
For example, training with TIN can improve the \OOD detection on CIFAR-100 compared to DTD based training while training on DTD provides perfect \OOD detection of MNIST dataset.
% However, on average the OOD detection performance is quite close for both OOD datasets in spite of the large difference in scale. This possibley suggests that a large collection of OOD data is not essential. 

%\paragraph{Benchmarks}
%Train on CIFAR10 (so far different ood datasets used for training): 
%Test on 6 datasets : Sun, CIFAR100, Places 50, INAT.
%Train on subset of CIFAR10, subset of CIFAR100 for ood
%Test on CIFAR100 another subset
%=================
%Get Energy-finetune with ResNet backbone. 

%\subsection{Ablations}
%Cross Entropy vs SupContt vs SupCon then CE.
%Show on CIFAR10 that SupContt with tinyimages


==> tables/baselines-cifar10-old.tex <==
\begin{table*}[t]
\footnotesize
\begin{center}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|}
\hline
Dataset/\Longunderstack{Method \\ Metrics} & \multicolumn{3}{c|}{\Longunderstack{CE \\ \\ FPR$\downarrow$ AUROC$\uparrow$  AUPR$\uparrow$ \\}} &  \multicolumn{3}{c|}{\Longunderstack{PSupCon \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{CE + Energy \\ \\ FPR$\downarrow$ AUROC$\uparrow$  AUPR$\uparrow$ \\}} & \multicolumn{3}{c|}{\Longunderstack{PSupCon + Energy \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon-R \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon-P \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}}
\\
\hline
\hline
\rowcolor{\fprcolor}
DTD & 25.01 & 95.02 & 98.81  
 & 14.09 & 97.44 & 99.44
&  7.83 & 98.43 & 99.67
 &  \textbf{2.71} & \textbf{99.43} & \textbf{99.87}
 &  5.26 & 99.00 & 99.79
 &  16.26 & 97.06 & 99.35
 \\ 


\rowcolor{\auroccolor}
SVHN & 3.08 & 99.19 & 99.84 
 & 3.16 & 99.39 & 99.87 
& 1.55 & 99.47 & 99.90
 & 1.92 & 99.57 & 99.91
 & \textbf{0.58} & \textbf{99.83} & \textbf{99.96}
 &  1.71 & 99.60 & 99.92
\\ 


\rowcolor{\fprcolor}
Places365 & 28.56 & 94.07 & 98.52 
& 26.96 & 94.88 & 98.79 
& 20.61 & 95.70 & 98.94 
& 36.85 & 92.11 & 98.07
& \textbf{20.17} & \textbf{95.89} & 98.96
 & 22.14 & 95.72 & \textbf{98.98}
\\ 


\rowcolor{\auroccolor}
LSUN-C & 12.10 & 97.68 & 99.54 
& 3.74 & 99.22 & 99.84 
& 5.28 & 98.75 & 99.75
& 64.98 & 81.89 & 95.42
 &  \textbf{1.38} & \textbf{99.63} & \textbf{99.93}
 &  1.73 & 99.53 & 99.91
\\ 


\rowcolor{\fprcolor}
LSUN-R & 8.98 & 98.15 & 99.63 
& 6.43 & 98.65 & 99.73 
& 8.69 & 98.37 & 99.67 
& \textbf{4.40} & \textbf{99.11} & \textbf{99.81}
 &  7.50 & 98.55 & 99.71
 &  6.23 & 98.72 & 99.74
\\ 


\rowcolor{\auroccolor}
iSUN & 11.54 & 97.86 & 99.58 
& 6.29 & 98.71 & 99.74 
& 7.24 & 98.59 & 99.72 
& \textbf{2.48} & \textbf{99.44} & \textbf{99.88}
 & 6.02 & 98.79 & 99.76
 & 6.53 & 98.76 & 99.75
\\ 


\rowcolor{\fprcolor}
iNaturalist & 37.24 & 94.10 & 98.77 
 & 10.70 & 98.18 & 99.63 
& 18.49 & 96.40 & 99.21
 & \textbf{7.53} & \textbf{98.61} & \textbf{99.70} 
 &  9.21 & 98.35 & 99.67 
 &   10.34 & 98.17 & 99.63\\ 


\rowcolor{\auroccolor}
CIFAR-100 & 40.73 & 91.85 & 98.03 
 & 41.03 & 92.30 & 98.19 
& 37.04 & 93.00 & 98.34
 & 51.07 & 89.59 & 97.57
 &  \textbf{35.41} & \textbf{93.22} & \textbf{98.39}
 &  39.97 & 92.66 & 98.34
\\ 


\rowcolor{\fprcolor}
Mnist & 30.88 & 95.76 & 99.17 
 & \textbf{1.62} & \textbf{99.50} & \textbf{99.90} 
& 32.55 & 94.93 & 98.97
 & 45.78 & 92.85 & 98.53
 &  3.86 & 99.37 & 99.87
 &  2.44 & 99.37 & 99.88
\\ 


\rowcolor{\auroccolor}
TIN & 32.05 & 93.22 & 98.30 
 & 30.95 & 93.86 & 98.50 
& 27.00 & 94.36 & 98.58
 &  31.80 & 93.45 & 98.47
 &  \textbf{25.85} & \textbf{94.49} & \textbf{98.61}
 &  27.80 & 94.38 & \textbf{98.61}
\\ 

\rowcolor{\fprcolor}
Average & 23.02 & 95.69 & 99.02 
 & 14.49 & 97.20 & 99.36 
& 16.63 & 96.80 & 99.27
 & 24.95 & 94.60 & 98.72
 &  \textbf{11.52} & \textbf{97.71} & \textbf{99.46} 
 &  13.51 & 97.39 & 99.41 \\ 
\hline
\end{tabular}}
\vspace{0.1cm}
\caption { \textbf{OOD detection performance on Cifar-10:} a) comparison of CE and PSupCon (1,2 columns) and, b) comparison of OOD training with our method compared to energy finetuning. Our method achieves the best performance  and improves over energy finetuning even when using pseudo OOD data.}
\label{tab:baselines_cifar10}
\end{center}
\end{table*}

==> tables/baselines-cifar10-older.tex <==
\begin{table*}[t]
\footnotesize
\begin{center}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|}
\hline
Dataset/\Longunderstack{Method \\ Metrics} & \multicolumn{3}{c|}{\Longunderstack{CE \\ \\ FPR$\downarrow$ AUROC$\uparrow$  AUPR$\uparrow$ \\}} & \multicolumn{3}{c|}{\Longunderstack{CE \\ (Energy) \\ FPR$\downarrow$ AUROC$\uparrow$  AUPR$\uparrow$ \\}} &  \multicolumn{3}{c|}{\Longunderstack{PSupCon \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{PSupCon \\ (Energy) \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon \\ Real \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon \\ Real (Energy) \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon \\ Pseudo \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon \\ Pseudo (Energy) \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}}
\\
\hline
\hline
\rowcolor{\fprcolor}
DTD & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!}  &   \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 14.09 & 97.44 & 99.44
 &  2.71 & 99.43 & 99.87
 &  5.26 & 99.00 & 99.79
 &  2.38 & 99.51 & 99.89
 &  16.26 & 97.06 & 99.35
 &  2.58 & 99.48 & 99.89
 \\ 


\rowcolor{\auroccolor}
SVHN & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 3.16 & 99.39 & 99.87 & 1.92 & 99.57 & 99.91
 &  0.58 & 99.83 & 99.96
 &  1.11 & 99.71 & 99.94
 &  1.71 & 99.60 & 99.92
 &  1.41 & 99.69 & 99.94
\\ 


\rowcolor{\fprcolor}
Places365 & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 26.96 & 94.88 & 98.79 & 36.85 & 92.11 & 98.07
 &  20.17 & 95.89 & 98.96
 &  36.86 & 92.20 & 98.12
 &  22.14 & 95.72 & 98.98
 &  35.49 & 92.49 & 98.17
\\ 


\rowcolor{\auroccolor}
LSUN-C & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 3.74 & 99.22 & 99.84 & 64.98 & 81.89 & 95.42
 &  1.38 & 99.63 & 99.93
 &  63.92 & 83.24 & 95.96
 &  1.73 & 99.53 & 99.91
 &  45.91 & 89.43 & 97.55
\\ 


\rowcolor{\fprcolor}
LSUN-R & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 6.43 & 98.65 & 99.73 & 4.40 & 99.11 & 99.81
 &  7.50 & 98.55 & 99.71
 &  6.31 & 98.73 & 99.73
 &  6.23 & 98.72 & 99.74
 &  2.22 & 99.50 & 99.90
\\ 


\rowcolor{\auroccolor}
iSUN & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & 6.29 & 98.71 & 99.74 & 2.48 & 99.44 & 99.88
 & 6.02 & 98.79 & 99.76
 & 4.17 & 99.09 & 99.81
 & 6.53 & 98.76 & 99.75
 & 1.33 & 99.70 & 99.94
\\ 


\rowcolor{\fprcolor}
iNaturalist & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 10.70 & 98.18 & 99.63 & 7.53 & 98.61 & 99.70&  9.21 & 98.35 & 99.67 &  7.51 & 98.54 & 99.68 &  10.34 & 98.17 & 99.63 &  6.38 & 98.78 & 99.74\\ 


\rowcolor{\auroccolor}
CIFAR-100 & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 41.03 & 92.30 & 98.19 & 51.07 & 89.59 & 97.57
 &  35.41 & 93.22 & 98.39
 &  49.19 & 90.09 & 97.72
 &  39.97 & 92.66 & 98.34
 &  49.34 & 89.65 & 97.57
\\ 


\rowcolor{\fprcolor}
Mnist & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 1.62 & 99.50 & 99.90 & 45.78 & 92.85 & 98.53
 &  3.86 & 99.37 & 99.87
 &  32.74 & 95.44 & 99.09
 &  2.44 & 99.37 & 99.88
 &  49.33 & 91.07 & 98.11
\\ 


\rowcolor{\auroccolor}
TIN & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 30.95 & 93.86 & 98.50 &  31.80 & 93.45 & 98.47
 &  25.85 & 94.49 & 98.61
 &  30.30 & 93.75 & 98.54
 &  27.80 & 94.38 & 98.61
 &  27.95 & 94.19 & 98.65
\\ 

\rowcolor{\fprcolor}
Average & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 14.49 & 97.20 & 99.36 & 24.95 & 94.60 & 98.72&  11.52 & 97.71 & 99.46 &  23.44 & 95.03 & 98.85  &  13.51 & 97.39 & 99.41 &  22.19 & 95.39 & 98.94 \\ 
\hline
\end{tabular}}
\vspace{0.1cm}
\caption {\textbf{Baselines on CIFAR-10:} 500 epochs.}
\label{tab:baselines_cifar10}
\end{center}
\vspace*{-0.5cm}
\end{table*}

==> tables/baselines-cifar100-old.tex <==
\begin{table*}[t]
\footnotesize
\begin{center}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|}
\hline
Dataset/\Longunderstack{Method \\ Metrics} & \multicolumn{3}{c|}{\Longunderstack{CE \\ \\ FPR$\downarrow$ AUROC$\uparrow$  AUPR$\uparrow$ \\}} & \multicolumn{3}{c|}{\Longunderstack{PSupCon \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{CE + Energy \\ \\ FPR$\downarrow$ AUROC$\uparrow$  AUPR$\uparrow$ \\}}  & \multicolumn{3}{c|}{\Longunderstack{PSupCon + Energy \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}}  & \multicolumn{3}{c|}{\Longunderstack{OPSupCon-R \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon-P \\ \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}}
\\
\hline
\hline
\rowcolor{\fprcolor}
DTD & 73.53 & 82.29 & 95.81
 & 66.14 & 80.14 & 94.53
 &   57.44 & 88.57 & 97.41
 &   \textbf{27.65} & \textbf{93.75} & \textbf{98.44}
&  50.10 & 88.16 & 97.20
 &  54.55 & 84.66 & 95.84
 \\ 


\rowcolor{\auroccolor}
SVHN & 34.38 & 93.89 & 98.71
 & 47.74 & 91.22 & 98.12
 & \textbf{17.21} & \textbf{96.93} & \textbf{99.34} 
 & 29.13 & 94.94 & 98.93
&  39.39 & 93.12 & 98.56
 &  51.86 & 90.76 & 98.02
\\ 


\rowcolor{\fprcolor}
Places365 & 80.83 & 77.96 & 94.52 
& 76.89 & 78.24 & 94.59
& 78.94 & 78.81 & 94.79 
 & 75.86 & 78.82 & 94.56
&  \textbf{74.22} & 79.33 & 94.83
 &  74.24 & \textbf{79.99} & \textbf{95.01}
\\ 


\rowcolor{\auroccolor}
LSUN-C & 54.84 & 90.19 & 97.93 
& 27.64 & 95.03 & 98.92
& 53.70 & 91.81 & 98.33 
 & 52.26 & 91.62 & 98.25
&  \textbf{18.34} & \textbf{96.65} & \textbf{99.30}
 &  19.46 & 96.51 & 99.25
\\ 


\rowcolor{\fprcolor}
LSUN-R & 62.42 & 88.00 & 97.42 
& 47.64 & 90.54 & 97.92
& 46.04 & 91.41 & 98.10 
 & \textbf{13.46} & \textbf{96.98} & \textbf{99.28}
&  40.86 & 91.97 & 98.23
 &  42.67 & 92.01 & 98.25
\\ 


\rowcolor{\auroccolor}
iSUN & 64.57 & 87.38 & 97.29 
& 55.10 & 88.29 & 97.38
& 50.00 & 90.33 & 97.85 
 & \textbf{14.38} & \textbf{96.92} & \textbf{99.29}
 & 49.07 & 90.24 & 97.86
 & 50.13 & 90.03 & 97.78
\\ 


\rowcolor{\fprcolor}
iNaturalist & 85.23 & 79.19 & 95.33 
& 43.67 & 89.11 & 97.24
& 79.15 & 83.25 & 96.32 
 & 70.28 & 85.19 & 96.71
& 41.00 & \textbf{90.16} & \textbf{97.58}
 &  \textbf{39.66} & 90.04 & 97.48\\ 


\rowcolor{\auroccolor}
CIFAR-10 & \textbf{76.84} & \textbf{79.16} & \textbf{94.88} 
& 83.45 & 73.12 & 92.66 
& 80.03 & 78.40 & 94.70 
& 89.84 & 71.60 & 92.75
&  84.41 & 70.52 & 91.27
 &  84.92 & 72.83 & 92.60
\\ 


\rowcolor{\fprcolor}
Mnist & 88.81 & 75.01 & 94.34 
& 33.93 & 94.24 & 98.79
& 95.33 & 67.34 & 92.36 
 & 96.27 & 77.41 & 95.21
&  32.67 & 94.73 & 98.91
 &  \textbf{26.49} & \textbf{95.87} & \textbf{99.14}
\\ 


\rowcolor{\auroccolor}
TIN & 75.20 & 80.56 & 95.08 
& 72.15 & 81.09 & 95.22
& 71.70 & 82.91 & 95.68 
 &  \textbf{62.50} & \textbf{85.02} & \textbf{96.17}
&  68.40 & 82.21 & 95.43
 &  70.70 & 81.78 & 95.37
\\ 

\rowcolor{\fprcolor}
Average & 69.67 & 83.36 & 96.13 
& 55.43 & 86.10 & 96.53 
& 62.95 & 84.98 & 96.49
& 53.16 & 87.22 & \textbf{96.96} 
&  \textbf{49.84} & \textbf{87.71} & 96.91 
&  51.46 & 87.44 & 96.87 \\ 
\hline
\end{tabular}}
\vspace{0.1cm}
\caption { \textbf{OOD detection performance on Cifar-100:} a) comparison of CE and PSupCon (1,2 columns) and, b) comparison of OOD training with our method compared to energy finetuning. Our method achieves the best performance  and improves over energy finetuning even when using pseudo OOD data.}
\label{tab:baselines_cifar100}
\end{center}
\end{table*}

==> tables/baselines-cifar100-older.tex <==
\begin{table*}[t]
\footnotesize
\begin{center}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|}
\hline
Dataset/\Longunderstack{Method \\ Metrics} & \multicolumn{3}{c|}{\Longunderstack{CE \\ FPR$\downarrow$ AUROC$\uparrow$  AUPR$\uparrow$ \\}} & \multicolumn{3}{c|}{\Longunderstack{CE + Energy \\ FPR$\downarrow$ AUROC$\uparrow$  AUPR$\uparrow$ \\}} & \multicolumn{3}{c|}{\Longunderstack{PSupCon \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{PSupCon + Energy \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}}  & \multicolumn{3}{c|}{\Longunderstack{OPSupCon Real \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon Real + Energy \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon Pseudo \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}} & \multicolumn{3}{c|}{\Longunderstack{OPSupCon Pseudo + Energy \\ FPR$\downarrow$ AUROC$\uparrow$  \AUPR$\uparrow$\\}}
\\
\hline
\hline
\rowcolor{\fprcolor}
DTD & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} &   \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 66.14 & 80.14 & 94.53
 &   27.65 & 93.75 & 98.44
&  50.10 & 88.16 & 97.20
 &  20.82 & 95.55 & 98.94
 &  54.55 & 84.66 & 95.84
 &  26.78 & 94.00 & 98.50
 \\ 


\rowcolor{\auroccolor}
SVHN & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 47.74 & 91.22 & 98.12
 & 29.13 & 94.94 & 98.93
&  39.39 & 93.12 & 98.56
 &  18.55 & 96.70 & 99.30
 &  51.86 & 90.76 & 98.02
 &  17.33 & 96.90 & 99.34
\\ 


\rowcolor{\fprcolor}
Places365 & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 76.89 & 78.24 & 94.59
 & 75.86 & 78.82 & 94.56
&  74.22 & 79.33 & 94.83
 &  77.35 & 77.62 & 94.15
 &  74.24 & 79.99 & 95.01
 &  74.75 & 78.82 & 94.45
\\ 


\rowcolor{\auroccolor}
LSUN-C & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 27.64 & 95.03 & 98.92
 & 52.26 & 91.62 & 98.25
&  18.34 & 96.65 & 99.30
 &  48.22 & 91.39 & 98.18
 &  19.46 & 96.51 & 99.25
 &  60.50 & 90.32 & 98.00
\\ 


\rowcolor{\fprcolor}
LSUN-R & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 47.64 & 90.54 & 97.92
 & 13.46 & 96.98 & 99.28
&  40.86 & 91.97 & 98.23
 &  10.21 & 97.84 & 99.50
 &  42.67 & 92.01 & 98.25
 &  12.86 & 97.32 & 99.38
\\ 


\rowcolor{\auroccolor}
iSUN & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & 55.10 & 88.29 & 97.38
 & 14.38 & 96.92 & 99.29
 & 49.07 & 90.24 & 97.86
 & 10.11 & 97.95 & 99.55
 & 50.13 & 90.03 & 97.78
 & 14.14 & 96.89 & 99.27
\\ 


\rowcolor{\fprcolor}
iNaturalist & \textbf{!!!} &  \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 43.67 & 89.11 & 97.24
 & 70.28 & 85.19 & 96.71
& 41.00 & 90.16 & 97.58 & 65.46 & 87.01 & 97.10
 &  39.66 & 90.04 & 97.48 &  71.69 & 83.86 & 96.34\\ 


\rowcolor{\auroccolor}
CIFAR-10 & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 83.45 & 73.12 & 92.66 & 89.84 & 71.60 & 92.75
&  84.41 & 70.52 & 91.27
 &  91.66 & 68.52 & 91.67
 &  84.92 & 72.83 & 92.60
 &  89.05 & 72.30 & 92.96
\\ 


\rowcolor{\fprcolor}
Mnist & \textbf{!!!} & \textbf{!!!}  & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 33.93 & 94.24 & 98.79
 & 96.27 & 77.41 & 95.21
&  32.67 & 94.73 & 98.91
 &  95.14 & 72.94 & 93.90
 &  26.49 & 95.87 & 99.14
 &  89.25 & 80.33 & 95.81
\\ 


\rowcolor{\auroccolor}
TIN & \textbf{!!!} & \textbf{!!!}  & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 72.15 & 81.09 & 95.22
 &  62.50 & 85.02 & 96.17
&  68.40 & 82.21 & 95.43
 &  61.10 & 85.11 & 96.20
 &  70.70 & 81.78 & 95.37
 &  61.20 & 85.39 & 96.23
\\ 

\rowcolor{\fprcolor}
Average & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} & \textbf{!!!} &  \textbf{!!!} & 55.43 & 86.10 & 96.53 & 53.16 & 87.22 & 96.96&  49.84 & 87.71 & 96.91 &  49.86 & 87.06 & 96.84  &  51.46 & 87.44 & 96.87 &  51.75 & 87.61 & 97.02 \\ 
\hline
\end{tabular}}
\vspace{0.1cm}
\caption {\textbf{Baselines on CIFAR-100:} 500 epochs.}
\label{tab:baselines_cifar100}
\end{center}
\vspace*{-0.7cm}
\end{table*}

==> tables/classification_accuracies.tex <==
%CIFAR10-SUPTT-Comparison to CE
\begin{table}[htbp]
\scriptsize
\centering
\begin{center}
%\begin{tabular}{|l|l l l|l l l|l l l|l l l|l l l|}
\begin{tabular}{|l|l|l|}
\hline
Method/Dataset & CIFAR-10 & CIFAR-100 \\
\hline
\hline
\rowcolor{\fprcolor}
CE & 95.36 & 76.64  \\

\rowcolor{\auroccolor}
%17.91  96.63  98.03
\SupTT & 95.28 & 76.82 \\
%4.74  99.04  98.10

\rowcolor{\fprcolor}
\oursreal & \textbf{95.66} & 76.83 \\
%27.42 & 94.65 & 48.84

\rowcolor{\auroccolor}
\oursfake  &  95.65 &  \textbf{78.16} \\
%1.18  99.67  99.69
\hline
\end{tabular}
\vspace{-0.2cm}
\caption {\scriptsize\textbf{ ID classification performance} Comparison of the classification accuracy ($\%$) on the ID task for the models in tables \ref{tab:baselines_cifar10} and~\ref{tab:baselines_cifar100}. Adding OOD regularization does not harm but rather improve the classification accuracy.}
\label{tab:cs_ac}
\end{center}
\vspace{-0.3cm}
\end{table}
